Federated Learning via Posterior Averaging: A New Perspective and Practical Algorithms

Federated learning is typically approached as an optimization problem, where the goal is to minimize a global loss function by distributing computation across client devices that possess local data and specify different parts of the global objective. We present an alternative perspective and formulate federated learning as a posterior inference problem, where the goal is to infer a global posterior distribution by having client devices each infer the posterior of their local data. While exact inference is often intractable, this perspective provides a principled way to search for global optima in federated settings. Further, starting with the analysis of federated quadratic objectives, we develop a computation- and communication-efficient approximate posterior inference algorithm -- federated posterior averaging (FedPA). Our algorithm uses MCMC for approximate inference of local posteriors on the clients and efficiently communicates their statistics to the server, where the latter uses them to refine a global estimate of the posterior mode. Finally, we show that FedPA generalizes federated averaging (FedAvg), can similarly benefit from adaptive optimizers, and yields state-of-the-art results on four realistic and challenging benchmarks, converging faster, to better optima.

==> tables/results_spicyfl.tex <==
\begin{table}[h]
    \vspace{-3ex}
    \caption{Comparison of \FedPA with baselines. %
    All metrics were computed on the evaluation sets and averaged over the last 100 rounds before the round limit was reached.
    The ``number of rounds to accuracy'' was determined based on the 10-round running average crossing the threshold for the first time.
    The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better.
    The best performance in each column is denoted in \best{bold}.}
    \vspace{-1ex}
    \small
    \begin{subtable}[t]{0.495\linewidth}
        \caption{\emnist}\vspace{-1ex}
        \begin{tabu} to \linewidth {X[2.2]|X[r]X[r]|X[0.8,r]X[0.8,r]}
            \toprule
                                                    & \multicolumn{2}{c|}{\textbf{accuracy (\%, $\uparrow$)}}   & \multicolumn{2}{c}{\textbf{rounds (\#, $\downarrow$)}}    \\
            \textbf{Method \,\textbackslash\, @}    & 500R          & 1500R                                     & 84\%              & 86\%                                  \\
            \midrule
            \AFO$^\dagger$                          & 80.4          & 86.8                                      & 546               & 1291                                  \\
            \MIME$^\ddagger$                         & 83.1         & *84.9                                     & 464               & *---                                  \\
            \midrule
            \FedAvg[1]                              & 83.9          & 86.5                                      & 451               & 1360                                  \\
            \FedAvg[M]                              & 85.8          & 85.9                                      & 86                & ---                                   \\
            \FedPA[M]                               & \best{86.5}   & \best{87.3}                               & \best{84}         & \best{92}                             \\
            \bottomrule
        \end{tabu}
        \label{tab:results-emnist}
        \vspace{1ex}
    \end{subtable}
    \begin{subtable}[t]{0.495\linewidth}
        \caption{\cifar}\vspace{-1ex}
        \begin{tabu} to \linewidth {X[2.2]|X[r]X[r]|X[0.8,r]X[0.8,r]}
            \toprule
                                                    & \multicolumn{2}{c|}{\textbf{accuracy (\%, $\uparrow$)}}   & \multicolumn{2}{c}{\textbf{rounds (\#, $\downarrow$)}}    \\
            \textbf{Method \,\textbackslash\, @}    & 1000R         & 1500R                                     & 30\%              & 40\%                                  \\
            \midrule
            \AFO$^\dagger$                          & 31.9          & 41.1                                      & 898               & 1401                                  \\
            \MIME$^\ddagger$                        & 33.2          & *33.9                                     & 680               & *---                                  \\
            \midrule
            \FedAvg[1]                              & 24.2          & 31.7                                      & 1379              & ---                                   \\
            \FedAvg[M]                              & 40.2          & 42.1                                      & \best{348}        & 896                                   \\
            \FedPA[M]                               & \best{44.3}   & \best{46.3}                               & \best{348}        & \best{543}                            \\
            \bottomrule
        \end{tabu}
        \label{tab:results-cifar}
        \vspace{1ex}
    \end{subtable}
    \label{tab:results}
    \\[-0.5ex]$^\dagger$ the best results taken from \citep{reddi2020adaptive}. $^\ddagger$ the best results taken from \citep{karimireddy2020mime}.\\
    * results were only available for the method trained up to 1000 rounds.
    \vspace{-2.5ex}
\end{table}

==> tables/results_spicyfl_app.tex <==
\begin{table}[t]
    \vspace{-2ex}
    \caption{Comparison of \FedPA with baselines. %
    All metrics were computed on the evaluation sets and averaged over the last 100 rounds before the round limit was reached.
    The ``number of rounds to accuracy'' was determined based on the 10-round running average crossing the threshold for the first time.
    The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better.
    The best performance in each column is denoted in \best{bold}.}
    \small
    \begin{subtable}[t]{\linewidth}
        \caption{\stackoverflow}
        \begin{tabu} to \linewidth {X[1.15]|X[1.1,r]X[0.9,r]|X[0.6,r]X[0.6,r]X[0.5,r]X[0.5,r]}
            \toprule
                                                        & \multicolumn{2}{c|}{\textbf{NWP}}                                             & \multicolumn{4}{c}{\textbf{LR (all metrics in \%, $\uparrow$)}}                   \\
            \textbf{Method \,\textbackslash\, Metric}   & \textbf{accuracy (\%, $\uparrow$)}    & \textbf{rounds (\#, $\downarrow$)}    & \textbf{precision}    & \textbf{recall@5} & \textbf{ma-F1}    & \textbf{mi-F1}    \\
            \midrule
            \AFO$^\dagger$                              & \best{23.4}                           & 1049                                  & ---                   & 68.0              & ---               & ---               \\
            \midrule
            \FedAvg[1]                                  & 22.8                                  & 1074                                  & 74.58                 & \best{69.1}       & 14.9              & 43.8              \\
            \FedAvg[M]                                  & 23.0                                  & 870                                   & \best{78.65}          & 68.7              & 15.6              & 43.3              \\
            \FedPA[M]                                   & \best{23.4}                           & \best{805}                            & 72.8                  & 68.6              & \best{17.3}       & \best{44.0}       \\
            \bottomrule
        \end{tabu}
        \label{tab:results-so-app}
    \end{subtable}
    \label{tab:results-app}
    \\[0.1ex]$^\dagger$ the best results taken from \citep{reddi2020adaptive}. $^\ddagger$ the best results taken from \citep{karimireddy2020mime}.\\
    * results were only available for the method trained to 1000 rounds.
\end{table}
